Deadlock-free routing for Full-mesh networks without using Virtual Channels

High-radix, low-diameter networks like HyperX and Dragonfly use a Full-mesh core, and rely on multiple virtual channels (VCs) to avoid packet deadlocks in adaptive routing. However, VCs introduce significant overhead in the switch in terms of area, power, and design complexity, limiting the switch scalability. This paper starts by revisiting VC-less routing through link ordering schemes in Full-mesh networks, which offer implementation simplicity but suffer from performance degradation under adversarial traffic. Thus, to overcome these challenges, we propose TERA (Topology-Embedded Routing Algorithm), a novel routing algorithm which employs an embedded physical subnetwork to provide deadlock-free non-minimal paths without using VCs. In a Full-mesh network, TERA outperforms link ordering routing algorithms by 80% when dealing with adversarial traffic, and up to 100% in application kernels. Furthermore, compared to other VC-based approaches, it reduces buffer requirements by 50%, while maintaining comparable latency and throughput. Lastly, early results from a 2D-HyperX evaluation show that TERA outperforms state-of-the-art algorithms that use the same number of VCs, achieving performance improvements of up to 32%.

==> dgfly_drawer.tex <==

%% dgfly drawer
\makeatletter
\newcommand{\dgflydraw}[6]{% #1=a, #2=b, #3=Delta_2, #4=t, #5=links, #6=width
	\xdef\a{#1}%
	\xdef\b{#2}%
	\xdef\Dg{#3}%
	\xdef\t{#4}%
	\pgfmathparse{360/\b}
	\global\let\gangle=\pgfmathresult
	%
	%\def\groupwidth{.3*#6}
	%\pgfmathsetlengthmacro{\groupwidth}{.3*#6}
	%\typeout{6=#6, b=\b}
	\pgfmathsetlengthmacro{\groupwidth}{1.3*#6/\b}%
	\pgfmathsetlengthmacro{\groupnodewidth}{\groupwidth+.2cm}%
	%\pgfmathparse{\groupwidth/\a}
	%\global\let\seprouters=\pgfmathresult
	\pgfmathsetlengthmacro{\seprouters}{\groupwidth/\a}%
	\pgfmathsetlengthmacro{\routernodewidth}{.9*\seprouters-1pt}%
	%\typeout{groupwidth=\groupwidth}
	%\typeout{seprouters=\seprouters}
	%\typein{}
	%\pgfmathparse{\seprouters/\Dg}
	%\global\let\sepchannels=\pgfmathresult
	%
	\pgfmathparse{int(\a-1)}
	\global\let\Pa=\pgfmathresult
	\pgfmathparse{int(\b-1)}
	\global\let\Pb=\pgfmathresult
	\pgfmathparse{int(\b-2)}
	\global\let\PPb=\pgfmathresult
	\pgfmathparse{int(\Dg-1)}
	\global\let\Pdg=\pgfmathresult
	\pgfmathparse{int(\t-1)}
	\global\let\Pt=\pgfmathresult
	\csname dgfly@configuration@#5\endcsname
	\typeout{DRAW!}%
	\begin{tikzpicture}[
		group/.style={densely dotted,draw,inner sep=0pt,rectangle,minimum width=\groupnodewidth,minimum height=.5*\groupnodewidth},
		router/.style={draw,rectangle,inner sep=0pt,minimum width=\routernodewidth,minimum height=.4*\groupnodewidth},
		%channel/.style={draw,circle,inner sep=0pt,minimum width=0.5*\sepchannels cm},
		link/.style={very thin},
		]%
	\foreach \ig in {0,...,\Pb}
	{
		\path ++(-90+\ig*\gangle:.35*#6) node[group,rotate=\ig*\gangle](group\ig)  {};
		\begin{scope}[transform shape,rotate=\gangle*\ig]
		\foreach \ia in {0,...,\Pa}
		{
			\path (group\ig) ++(0:{0.5*\seprouters-0.5*\a*\seprouters}) ++(\ia*\seprouters,0) node[router](router\ig_\ia) {};
			\expandafter\xdef\csname style\ig_\ia\endcsname{}
		}
		\pgfmathparse{int(\a-2)}
		\let\PPa=\pgfmathresult
		\foreach \ia in {0,...,\PPa}
		{
			\pgfmathparse{int(\ia+1)}
			\let\sia=\pgfmathresult
			\foreach \ja in {\sia,...,\Pa}
			{
				\draw[link] (router\ig_\ia) edge[out=-90,in=-90] (router\ig_\ja);
			}
		}
		\end{scope}
	}
	\foreach \ia in {0,...,\Pa}
	\foreach \ih in {0,...,\Pdg}
	{
		\expandafter\xdef\csname style0_\ia_\ih\endcsname{very thick}
		\expandafter\xdef\csname style0_\ia\endcsname{very thick}
	}
	\foreach \ig in {0,...,\Pb}
	{
		\foreach \ia in {0,...,\Pa}
		{
			\foreach \ih in {0,...,\Pdg}
			{
				%\palmtreelink{\ig}{\ia}{\ih}
				%\tablelink{\ig}{\ia}{\ih}
				\dgflylink{\ig}{\ia}{\ih}
				%
				%\ifthenelse{\resultb<0}{}
				%{
				%	\draw[link,
				%		\csname style\ig_\ia\endcsname,
				%		\csname style\resultb_\resulta\endcsname,
				%		] (router\ig_\ia) -- (router\resultb_\resulta);
				%}
				\ifthenelse{\resultb>\ig}
				{
					\pgfmathparse{90+(\ig+.5*(\ih+.5-.5*\Dg)/\Dg)*\gangle}
					\let\aangle=\pgfmathresult
					%\pgfmathparse{90+\resultb*\gangle}
					\pgfmathparse{90+(\resultb-.5*(\ih+.5-.5*\Dg)/\Dg)*\gangle}
					\let\bangle=\pgfmathresult
					\draw[link,
						\csname style\ig_\ia\endcsname,
						\csname style\resultb_\resulta\endcsname,
						] (router\ig_\ia) edge[out=\aangle,in=\bangle] (router\resultb_\resulta);
				}{}
			}
		}
	}
	%\draw[red] (current bounding box.north west) rectangle (current bounding box.south east);
	\end{tikzpicture}
}


\newcommand{\dgflyplusdraw}[6]{% #1=a, #2=b, #3=Delta_2, #4=t, #5=links, #6=width
	\xdef\a{#1}%
	\xdef\b{#2}%
	\xdef\Dg{#3}%
	\xdef\t{#4}%
	\pgfmathparse{360/\b}
	\global\let\gangle=\pgfmathresult
	%
	%\def\groupwidth{.3*#6}
	%\pgfmathsetlengthmacro{\groupwidth}{.3*#6}
	%\typeout{6=#6, b=\b}
	\pgfmathsetlengthmacro{\groupwidth}{1.3*#6/\b}%
	\pgfmathsetlengthmacro{\groupnodewidth}{\groupwidth+.2cm}%
	%\pgfmathparse{\groupwidth/\a}
	%\global\let\seprouters=\pgfmathresult
	\pgfmathsetlengthmacro{\seprouters}{\groupwidth/\a}%
	\pgfmathsetlengthmacro{\routernodewidth}{.9*\seprouters-1pt}%
	%\typeout{groupwidth=\groupwidth}
	%\typeout{seprouters=\seprouters}
	%\typein{}
	%\pgfmathparse{\seprouters/\Dg}
	%\global\let\sepchannels=\pgfmathresult
	%
	\pgfmathparse{int(\a-1)}
	\global\let\Pa=\pgfmathresult
	\pgfmathparse{int(\b-1)}
	\global\let\Pb=\pgfmathresult
	\pgfmathparse{int(\b-2)}
	\global\let\PPb=\pgfmathresult
	\pgfmathparse{int(\Dg-1)}
	\global\let\Pdg=\pgfmathresult
	\pgfmathparse{int(\t-1)}
	\global\let\Pt=\pgfmathresult
	\csname dgfly@configuration@#5\endcsname
	\typeout{DRAW!}%
	\begin{tikzpicture}[
		group/.style={densely dotted,draw,inner sep=0pt,rectangle,minimum width=\groupnodewidth,minimum height=\groupnodewidth},
		router/.style={draw,rectangle,inner sep=0pt,minimum width=\routernodewidth,minimum height=.2*\groupnodewidth},
		%channel/.style={draw,circle,inner sep=0pt,minimum width=0.5*\sepchannels cm},
		link/.style={very thin},
		]%
	\foreach \ig in {0,...,\Pb}
	{
		\path ++(-90+\ig*\gangle:.35*#6) node[group,rotate=\ig*\gangle](group\ig)  {};
		\begin{scope}[transform shape,rotate=\gangle*\ig]
		\foreach \ia in {0,...,\Pa}
		{
			\path (group\ig) ++(0:{0.5*\seprouters-0.5*\a*\seprouters}) ++(\ia*\seprouters,.3*\groupnodewidth) node[router](router\ig_\ia) {};
			\path (group\ig) ++(0:{0.5*\seprouters-0.5*\a*\seprouters}) ++(\ia*\seprouters,-.3*\groupnodewidth) node[router](leaf\ig_\ia) {};
			\expandafter\xdef\csname style\ig_\ia\endcsname{}
		}
		\end{scope}
	}
	\foreach \ia in {0,...,\Pa}
	\foreach \ih in {0,...,\Pdg}
	{
		\expandafter\xdef\csname style0_\ia_\ih\endcsname{very thick}
		\expandafter\xdef\csname style0_\ia\endcsname{very thick}
	}
	\foreach \ig in {0,...,\Pb}
	{
		\foreach \ia in {0,...,\Pa}
		{
			\foreach \ih in {0,...,\Pdg}
			{
				%\palmtreelink{\ig}{\ia}{\ih}
				%\tablelink{\ig}{\ia}{\ih}
				\dgflylink{\ig}{\ia}{\ih}
				%
				%\ifthenelse{\resultb<0}{}
				%{
				%	\draw[link,
				%		\csname style\ig_\ia\endcsname,
				%		\csname style\resultb_\resulta\endcsname,
				%		] (router\ig_\ia) -- (router\resultb_\resulta);
				%}
				\ifthenelse{\resultb>\ig}
				{
					\pgfmathparse{90+(\ig+.5*(\ih+.5-.5*\Dg)/\Dg)*\gangle}
					\let\aangle=\pgfmathresult
					%\pgfmathparse{90+\resultb*\gangle}
					\pgfmathparse{90+(\resultb-.5*(\ih+.5-.5*\Dg)/\Dg)*\gangle}
					\let\bangle=\pgfmathresult
					\draw[link,
						\csname style\ig_\ia\endcsname,
						\csname style\resultb_\resulta\endcsname,
						] (router\ig_\ia) edge[out=\aangle,in=\bangle] (router\resultb_\resulta);
				}{}
			}
			\foreach \ja in {0,...,\Pa}
			{
				\draw[link] (router\ig_\ia) -- (leaf\ig_\ja);
			}
		}
	}
	%\draw[red] (current bounding box.north west) rectangle (current bounding box.south east);
	\end{tikzpicture}
}


\newcommand{\dgflydrawrect}[6]{% #1=a, #2=b, #3=Delta_2, #4=t, #5=links, #6=width
	\xdef\a{#1}%
	\xdef\b{#2}%
	\xdef\Dg{#3}%
	\xdef\t{#4}%
	\pgfmathparse{360/\b}
	\global\let\gangle=\pgfmathresult
	%
	%\def\groupwidth{.3*#6}
	%\pgfmathsetlengthmacro{\groupwidth}{.3*#6}
	%\typeout{6=#6, b=\b}
	%\pgfmathsetlengthmacro{\groupwidth}{1.3*#6/\b}%
	\pgfmathsetlengthmacro{\groupwidth}{#6}%
	\pgfmathsetlengthmacro{\groupnodewidth}{\groupwidth+.2cm}%
	\pgfmathsetlengthmacro{\groupnodeheight}{\groupwidth/\b}%
	%\pgfmathparse{\groupwidth/\a}
	%\global\let\seprouters=\pgfmathresult
	\pgfmathsetlengthmacro{\seprouters}{\groupwidth/\a}%
	\pgfmathsetlengthmacro{\routernodewidth}{.5*\seprouters-1pt}%
	%\typeout{groupwidth=\groupwidth}
	%\typeout{seprouters=\seprouters}
	%\typein{}
	%\pgfmathparse{\seprouters/\Dg}
	%\global\let\sepchannels=\pgfmathresult
	%
	\pgfmathparse{int(\a-1)}
	\global\let\Pa=\pgfmathresult
	\pgfmathparse{int(\b-1)}
	\global\let\Pb=\pgfmathresult
	\pgfmathparse{int(\b-2)}
	\global\let\PPb=\pgfmathresult
	\pgfmathparse{int(\Dg-1)}
	\global\let\Pdg=\pgfmathresult
	\pgfmathparse{int(\t-1)}
	\global\let\Pt=\pgfmathresult
	\csname dgfly@configuration@#5\endcsname
	\typeout{DRAW!}%
	\begin{tikzpicture}[
		group/.style={very thick,,inner sep=0pt,rectangle,minimum width=\groupnodewidth,minimum height=\groupnodeheight},
		router/.style={draw,rectangle,inner sep=0pt,minimum width=\routernodewidth,minimum height=.6*\groupnodeheight},
		%channel/.style={draw,circle,inner sep=0pt,minimum width=0.5*\sepchannels cm},
		link/.style={very thin},
		]%
	\foreach \ig in {0,...,\Pb}
	{
		%\path ++(-90+\ig*\gangle:.35*#6) node[group,rotate=\ig*\gangle](group\ig)  {};
		\path ++(0,\ig*\groupnodeheight) node[group](group\ig)  {};
		%\begin{scope}[transform shape,rotate=\gangle*\ig]
		\begin{scope}
		\foreach \ia in {0,...,\Pa}
		{
			\path (group\ig) ++(0:{0.5*\seprouters-0.5*\a*\seprouters}) ++(\ia*\seprouters,0) node[router](router\ig_\ia) {};
			\expandafter\xdef\csname style\ig_\ia\endcsname{}
		}
		\end{scope}
	}
	\foreach \ia in {0,...,\Pa}
	\foreach \ih in {0,...,\Pdg}
	{
		\expandafter\xdef\csname style0_\ia_\ih\endcsname{very thick}
		\expandafter\xdef\csname style0_\ia\endcsname{very thick}
	}
	\foreach \ig in {0,...,\Pb}
	{
		\foreach \ia in {0,...,\Pa}
		{
			\foreach \ih in {0,...,\Pdg}
			{
				%\palmtreelink{\ig}{\ia}{\ih}
				%\tablelink{\ig}{\ia}{\ih}
				\dgflylink{\ig}{\ia}{\ih}
				%
				%\ifthenelse{\resultb<0}{}
				%{
				%	\draw[link,
				%		\csname style\ig_\ia\endcsname,
				%		\csname style\resultb_\resulta\endcsname,
				%		] (router\ig_\ia) -- (router\resultb_\resulta);
				%}
				\ifthenelse{\resultb>\ig}
				{
					\draw[link,
						\csname style\ig_\ia\endcsname,
						\csname style\resultb_\resulta\endcsname,
						] (router\ig_\ia) edge[in=0,out=0,looseness=0.3] (router\resultb_\resulta);
				}{}
			}
		}
	}
	%intragroup links
	\pgfmathparse{int(\a-2)}
	\global\let\PPa=\pgfmathresult
	\foreach \ig in {0,...,\Pb}
	{
		\foreach \ia in {0,...,\PPa}
		{
			\pgfmathparse{int(\ia+1)}
			\global\let\Sia=\pgfmathresult
			\foreach \na in {\Sia,...,\Pa}
			{
				\draw[link,
					] (router\ig_\ia) edge[in=-90,out=-90,looseness=0.3] (router\ig_\na);
			}
		}
	}
	%\draw[red] (current bounding box.north west) rectangle (current bounding box.south east);
	\end{tikzpicture}
}
\newcommand{\palmtree@link}[3]{%
	\edef\ig{#1}
	\edef\ia{#2}
	\edef\ih{#3}
	\pgfmathparse{int(\a-\ia-1)}
	\xdef\resulta{\pgfmathresult}
	\pgfmathparse{int(mod(\ig+1+mod(\resulta*\Dg+\ih,\b-1),\b))}
	\xdef\resultb{\pgfmathresult}
}
\newcommand\dgfly@configuration@palmtree{%
	\global\let\dgflylink=\palmtree@link
}
\newcommand{\tablelink}[3]{%
	\xdef\resulta{\csname linksa#1_#2_#3\endcsname}
	\xdef\resultb{\csname linksb#1_#2_#3\endcsname}
}
\newcommand\dgfly@configuration@random{%
	\global\let\dgflylink=\tablelink
	\foreach \ib in {0,...,\Pb}
	\foreach \ia in {0,...,\Pa}
	\foreach \idg in {0,...,\Pdg}
	{%
		%\typeout{assigned\ib_\ia_\idg:=-1}
		\expandafter\xdef\csname assigned\ib_\ia_\idg\endcsname{-1}%
	}%
	\foreach \xb in {0,...,\PPb}
	{%
	\pgfmathtruncatemacro\Nxb{\xb+1}%
	\foreach \yb in {\Nxb,...,\Pb}
	\foreach \ti in {1,...,\t}
	{%
		\loop%
			\pgfmathrandominteger{\xia}{0}{\Pa}%
			\pgfmathrandominteger{\xidg}{0}{\Pdg}%
			\xdef\xia{\xia}%
			\xdef\xidg{\xidg}%
			\edef\x{\csname assigned\xb_\xia_\xidg\endcsname}%
			\ifnum \x>-1%
			\repeat%
		%\typeout{assigned\xb_\xia_\xidg:=\yb}%
		\expandafter\xdef\csname assigned\xb_\xia_\xidg\endcsname{\yb}%
		\expandafter\xdef\csname bridge_router\xb_\yb\endcsname{\xia}%
		\expandafter\xdef\csname linksb\xb_\xia_\xidg\endcsname{\yb}%XXX%
		%%%%%%%%%%%%%%%%%%%%%%%%%
		\loop%
			\pgfmathrandominteger{\yia}{0}{\Pa}%
			\pgfmathrandominteger{\yidg}{0}{\Pdg}%
			\xdef\yia{\yia}%
			\xdef\yidg{\yidg}%
			\edef\x{\csname assigned\yb_\yia_\yidg\endcsname}%
			\ifnum \x>-1%
			\repeat%
		\expandafter\xdef\csname assigned\yb_\yia_\yidg\endcsname{\xb}%
		\expandafter\xdef\csname bridge_router\yb_\xb\endcsname{\yia}%
		\expandafter\xdef\csname linksb\yb_\yia_\yidg\endcsname{\yb}%XXX%
		%%
		\expandafter\xdef\csname linksa\xb_\xia_\xidg\endcsname{\yia}%
		\expandafter\xdef\csname linksa\yb_\yia_\yidg\endcsname{\xia}%
	}%
	}%
}
\newcommand{\cycles@link}[3]{%
	\edef\ig{#1}
	\edef\ia{#2}
	\edef\ih{#3}
	\xdef\resulta{\ia}
	\ifnum\ih=1
		\pgfmathparse{int(mod(\ig+\ia+1,\b))}
	\else
		\pgfmathparse{int(mod(\b+\ig-\ia-1,\b))}
	\fi
	\xdef\resultb{\pgfmathresult}
}
\newcommand\dgfly@configuration@cycles{%
	\ifnum\Dg=2\relax\else\errmessage{This configuration requires global degree 2}\fi
	\global\let\dgflylink=\cycles@link
}
\newcommand{\hamming@link}[3]{%
	\edef\ig{#1}
	\edef\ia{#2}
	\edef\ih{#3}
	\xdef\resulta{\ia}
	\pgfmathparse{int(mod(\ig+\ih+1,\b))}
	%\ifnum\ih=1
	%	\pgfmathparse{int(mod(\ig+\ia+1,\b))}
	%\else
	%	\pgfmathparse{int(mod(\b+\ig-\ia-1,\b))}
	%\fi
	\xdef\resultb{\pgfmathresult}
}
\newcommand\dgfly@configuration@hamming{%
	\ifnum\a=\t\relax\else\errmessage{}\fi
	\global\let\dgflylink=\hamming@link
}
\newcommand{\consecutive@link}[3]{%
	\edef\ig{#1}
	\edef\ia{#2}
	\edef\ih{#3}
	\pgfmathparse{int(\ia*\Dg+\ih)}
	\let\G=\pgfmathresult
	%\typeout{ig=\ig\ ia=\ia\ ih=\ih\ G=\G}
	\ifnum \G<\ig\relax
		\pgfmathparse{int(floor((\ig-1)/\Dg))}
		\xdef\resulta{\pgfmathresult}
		\xdef\resultb{\G}
	\else
		\pgfmathparse{int(floor((\ig)/\Dg))}
		\xdef\resulta{\pgfmathresult}
		\pgfmathparse{int(\G+1)}
		\xdef\resultb{\pgfmathresult}
	\fi
}
\newcommand\dgfly@configuration@consecutive{%
	\global\let\dgflylink=\consecutive@link
}
\makeatother

